Heuristics for Network Coding in Wireless Networks

Multicast is a central challenge for emerging multi-hop wireless architectures such as wireless mesh networks, because of its substantial cost in terms of bandwidth. In this report, we study one specific case of multicast: broadcasting, sending data from one source to all nodes, in a multi-hop wireless network. The broadcast we focus on is based on network coding, a promising avenue for reducing cost; previous work of ours showed that the performance of network coding with simple heuristics is asymptotically optimal: each transmission is beneficial to nearly every receiver. This is for homogenous and large networks of the plan. But for small, sparse or for inhomogeneous networks, some additional heuristics are required. This report proposes such additional new heuristics (for selecting rates) for broadcasting with network coding. Our heuristics are intended to use only simple local topology information. We detail the logic of the heuristics, and with experimental results, we illustrate the behavior of the heuristics, and demonstrate their excellent performance.

==> Makefile <==
#---------------------------------------------------------------------------
# Makefile for report
#---------------------------------------------------------------------------


IMG=lattice-es random-es \
 random-torus \
lattice-IRON                 rap-rech1.pdf \
random-uniform \
lattice-irms    \
random-irms \
mincut-cmu-dis \
mincut-mu-dis \
cost-random-200_WO  \
cost-random-M20   \
rel-eff \
Logo-INRIA-couleur.pdf  \
rap-tech.pdf \
Logo-INRIA-picto.pdf     \
 Logo-INRIA-Rocq-couleur.pdf \
 sparse_ununiform_net \
cost-random-400              cost-random-800 \
cost-random-torus-200_WO  \
cost-random-torus-400 \
rap-rech1.ps \
Logo-INRIA-picto.ps    \
 Logo-INRIA-Rocq-couleur.ps \
 Logo-INRIA-couleur.ps

#---------------------------------------------------------------------------

TARGET=rr.pdf

all: ${TARGET}


pdf: rr.pdf

rr.ps: rr.tex
	pslatex rr.tex
	pslatex rr.tex
	dvips -o rr.ps rr.dvi

rr.pdf: rr.tex ${IMG}
	pdflatex rr.tex
	pdflatex rr.tex

%.pdf: %.ps ; epstopdf $<
%.pdf: %.eps ; epstopdf $<

#---------------------------------------------------------------------------

RRNAME=HeuristicsNetCod
RRVER=1.0.2

PKGFILELIST=RR.sty algorithm2e.sty simplemargins.sty preamble.tex Makefile \
           ${IMG}

RRpkg:
	mkdir tmp || true
	rm -rf tmp/${RRNAME}-${RRVER}
	mkdir tmp/${RRNAME}-${RRVER}
	cp -av rr.tex \
	       tmp/${RRNAME}-${RRVER}/${RRNAME}.tex
	for SUFFIX in "" .eps .pdf ; do \
	   for DIR in . Graph ; do for i in ${PKGFILELIST} ; do \
	  test -e $${DIR}/$$i$${SUFFIX} \
	    && cp $${DIR}/$$i$${SUFFIX} tmp/${RRNAME}-${RRVER} ||true;\
	done ; done ; done
	(cd tmp && tar czvf ${RRNAME}-${RRVER}.tar.gz ${RRNAME}-${RRVER})
	cd tmp/${RRNAME}-${RRVER} && pdflatex ${RRNAME} && pdflatex ${RRNAME}

#---------------------------------------------------------------------------

